Assisted Living in the United States: an Open Dataset

An assisted living facility (ALF) is a place where someone can live, have access to social supports such as transportation, and receive assistance with the activities of daily living such as toileting and dressing. Despite the important role of ALFs, they are not required to be certified with Medicare and there is no public national database of these facilities. We present the first public dataset of ALFs in the United States, covering all 50 states and DC with 44,638 facilities and over 1.2 million beds. This dataset can help provide answers to existing public health questions as well as help those in need find a facility. The dataset was validated by replicating the results of a nationwide study of ALFs that uses closed data [4], where the prevalence of ALFs is assessed with respect to county-level socioeconomic variables related to health disparity such as race, disability, and income. To showcase the value of this dataset, we also propose a novel metric to assess access to community-based care. We calculate the average distance an individual in need must travel in order to reach an ALF. The dataset and all relevant code are available at github.com/antonstengel/assisted-living-data.

==> images/teximage.tex <==
\frame{\begin{picture}(100,100)
\put(25,50){\dashbox{.5}(10,10){$A$}}
\put(50,50){\dashbox{.5}(10,10){$B$}}
\end{picture}}


==> table_county_variables.tex <==
\begin{table}[h!]
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{l}
\toprule
Variable
\\
\midrule
Median age \\
Percent of population 65 or older  \\
Percent of population 85 or older  \\
Less than high school  \\
College education or higher  \\
Median household income (\$1000s)  \\
Unemployment rate  \\
Poverty rate \\
Home ownership rate \\
Median home value of owned homes (\$1000s) \\
Percent white population  \\
Percent black population \\
Percent hispanic population   \\
\bottomrule
\end{tabular}
}
\vspace{1ex}
\caption{\textbf{Variables associated with every United States County, drawn from \cite{bureau_sample_nodate}.}}
\label{table:county-variables}
\end{table}
